Deep Learning COVID-19 Features on CXR using Limited Training Data Sets

Under the global pandemic of COVID-19, the use of artificial intelligence to analyze chest X-ray (CXR) image for COVID-19 diagnosis and patient triage is becoming important. Unfortunately, due to the emergent nature of the COVID-19 pandemic, a systematic collection of the CXR data set for deep neural network training is difficult. To address this problem, here we propose a patch-based convolutional neural network approach with a relatively small number of trainable parameters for COVID-19 diagnosis. The proposed method is inspired by our statistical analysis of the potential imaging biomarkers of the CXR radiographs. Experimental results show that our method achieves state-of-the-art performance and provides clinically interpretable saliency maps, which are useful for COVID-19 diagnosis and patient triage.

==> packages.tex <==
% packages.tex
% load a lot of possibly useful packages
% all of these are documented on web sites online

\usepackage{outline}
\usepackage{pmgraph}
\usepackage[normalem]{ulem}
\usepackage[utf8]{inputenc}
%\usepackage{gensymb}
\usepackage{amssymb}
\usepackage{hyperref}
\usepackage{amsmath}
\usepackage{graphicx}
%\usepackage[text={6.5in,9in},centering]{geometry}
%%%
\usepackage{times}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage[colorinlistoftodos]{todonotes} % for \todo
\usepackage{cite}
\usepackage{bm} % bold
%\setlength{\parskip}{1em}
%\setlength{\parindent}{0em}
%%%
%\usepackage[font=footnotesize,labelfont=bf]{caption}
%\usepackage[font=footnotesize,labelfont=bf]{subcaption}
%\usepackage{subcaption}
\usepackage{url}

\usepackage{epstopdf}
%\epstopdfDeclareGraphicsRule{.tiff}{png}{.png}{convert #1 \OutputFile}
%\AppendGraphicsExtensions{.tiff}
%\graphicspath{{fig/}} % Directory in which figures are stored

\usepackage{epsfig}
\usepackage{tikz}
\usetikzlibrary{spy}
\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{mathrsfs}

\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{booktabs}       % professional-quality tables

%% Sungjoon

\usepackage{amsmath,graphicx,caption,mathtools,amssymb,amsthm}
\usepackage{graphicx}
\usepackage{multirow}
%\usepackage{subcaption}
\usepackage{accents}
%\usepackage{txfonts}
% \usepackage{eucal}

%\addbibresource{refs_jcy.bib}
